Optimization-Based On-Road Path Planning for Articulated Vehicles

Maneuvering an articulated vehicle on narrow road stretches is often a challenging task for a human driver. Unless the vehicle is accurately steered, parts of the vehicle's bodies may exceed its assigned drive lane, resulting in an increased risk of collision with surrounding traffic. In this work, an optimization-based path-planning algorithm is proposed targeting on-road driving scenarios for articulated vehicles composed of a tractor and a trailer. To this end, we model the tractor-trailer vehicle in a road-aligned coordinate frame suited for on-road planning. Based on driving heuristics, a set of different optimization objectives is proposed, with the overall goal of designing a path planner that computes paths which minimize the off-track of the vehicle bodies swept area, while remaining on the road and avoiding collision with obstacles. The proposed optimization-based path-planning algorithm, together with the different optimization objectives, is evaluated and analyzed in simulations on a set of complicated and practically relevant on-road planning scenarios using the most challenging tractor-trailer dimensions.

==> figures/tikz/draw_length_measure.tex <==
% This file defines the draw length measure command

\newcommand{\DrawLengthMeasure}[6]{
% #1 Start x
% #2 Start y
% #3 Final x
% #4 Final y
% #5 Measure angle (inferable from previous arguments, but easier if I just receive it )
% #6 Text to place

\coordinate (StartPoint) at ($(#1, #2)$);
\coordinate (FinalPoint) at ($(#3, #4)$);
%\coordinate (CornerFL) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*#4}, {sin(#3)*#5+cos(#3)*#4})$);

\draw[fill=gray] (StartPoint) -- (FinalPoint);

\def\TickHalfLength{0.1}
\coordinate (StartPointA) at ($(#1, #2) + ({\TickHalfLength*cos(#5+90)},{\TickHalfLength*sin(#5+90)})$);
\coordinate (StartPointB) at ($(#1, #2) + ({\TickHalfLength*cos(#5-90)},{\TickHalfLength*sin(#5-90)})$);
\draw[fill=gray] (StartPointA) -- (StartPointB);

\coordinate (FinalPointA) at ($(#3, #4) + ({\TickHalfLength*cos(#5+90)},{\TickHalfLength*sin(#5+90)})$);
\coordinate (FinalPointB) at ($(#3, #4) + ({\TickHalfLength*cos(#5-90)},{\TickHalfLength*sin(#5-90)})$);
\draw[fill=gray] (FinalPointA) -- (FinalPointB);

\def\ExtraOffsetX{0.25*cos(#5+90)}
\def\ExtraOffsetY{0.25*sin(#5+90)}

\node[] at ($(StartPoint)!0.5!(FinalPoint) + ({\ExtraOffsetX}, {\ExtraOffsetY})$) {#6};  
%\draw[] (\ReferenceOriginX,\ReferenceOriginY)--(1.5,\ReferenceOriginY) node[right]{$x$};

}

==> figures/tikz/draw_side_metric.tex <==
% This file defines the draw vehicle command

\newcommand{\DrawSideMetric}[8]{
% #1 Center x
% #2 Center y
% #3 Orientation
% #4 Length up
% #5 Length down
% #6 Text up
% #7 Text down
% #8 Text lateral offset

\coordinate (CenterMetric) at (#1, #2);
\coordinate (TopLength) at ($ (CenterMetric) + ({cos(#3+90)*#4}, {sin(#3+90)*#4})$);
\coordinate (DownLength) at ($ (CenterMetric) + ({cos(#3-90)*#5}, {sin(#3-90)*#5})$);

\node[blue] at ($(CenterMetric)!0.5!(TopLength) + (#8, 0)$) {#6};
\node[red] at ($(CenterMetric)!0.5!(DownLength) + (#8, 0)$) {#7};

\draw[\ReferencePathColor,thick] (CenterMetric) circle (1pt);
\draw [->, thick, blue] (CenterMetric) -- (TopLength);
\draw [->, thick, red] (CenterMetric) -- (DownLength);

}

==> figures/tikz/draw_trailer.tex <==
% This file defines the draw vehicle command

\newcommand{\DrawTrailer}[6]{
% #1 Vehicle x
% #2 Vehicle y
% #3 Vehicle theta
% #4 Vehicle half width
% #5 Vehicle front length
% #6 Vehicle rear length

\coordinate (CornerFR) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*-#4}, {sin(#3)*#5+cos(#3)*-#4})$);
\coordinate (CornerFL) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*#4}, {sin(#3)*#5+cos(#3)*#4})$);
\coordinate (CornerRL) at ($ (#1, #2) + ({cos(#3)*-#6-sin(#3)*#4}, {sin(#3)*-#6+cos(#3)*#4})$);
\coordinate (CornerRR) at ($ (#1, #2) + ({cos(#3)*-#6-sin(#3)*-#4}, {sin(#3)*-#6+cos(#3)*-#4})$);

\draw[fill=gray,very thick, fill opacity=0.4] (CornerFL) -- (CornerFR) -- (CornerRR) -- (CornerRL) -- cycle;


\def\AxleLength{#5-#6}

\coordinate (WheelRL) at ($ (#1, #2) + ({-sin(#3)*#4}, {cos(#3)*#4})$);
\coordinate (WheelRR) at ($ (#1, #2) + ({-sin(#3)*-#4}, {cos(#3)*-#4})$);

\def\WheelWidth{0.06}
\def\WheelHeight{0.125}

\DrawWheel{(WheelRL)}{#3}{\WheelWidth}{\WheelHeight}
\DrawWheel{(WheelRR)}{#3}{\WheelWidth}{\WheelHeight}


}

==> figures/tikz/draw_vehicle.tex <==
% This file defines the draw vehicle command

\newcommand{\DrawVehicle}[6]{
% #1 Vehicle x
% #2 Vehicle y
% #3 Vehicle theta
% #4 Vehicle half width
% #5 Vehicle front length
% #6 Vehicle rear length

\coordinate (CornerFR) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*-#4}, {sin(#3)*#5+cos(#3)*-#4})$);
\coordinate (CornerFL) at ($ (#1, #2) + ({cos(#3)*#5-sin(#3)*#4}, {sin(#3)*#5+cos(#3)*#4})$);
\coordinate (CornerRL) at ($ (#1, #2) + ({cos(#3)*-#6-sin(#3)*#4}, {sin(#3)*-#6+cos(#3)*#4})$);
\coordinate (CornerRR) at ($ (#1, #2) + ({cos(#3)*-#6-sin(#3)*-#4}, {sin(#3)*-#6+cos(#3)*-#4})$);

\draw[fill=gray,very thick, fill opacity=0.4] (CornerFL) -- (CornerFR) -- (CornerRR) -- (CornerRL) -- cycle;


\def\AxleLength{#5-#6}

\coordinate (WheelFR) at ($ (#1, #2) + ({cos(#3)*(\AxleLength)-sin(#3)*-#4}, {sin(#3)*(\AxleLength)+cos(#3)*-#4})$);
\coordinate (WheelFL) at ($ (#1, #2) + ({cos(#3)*(\AxleLength)-sin(#3)*#4}, {sin(#3)*(\AxleLength)+cos(#3)*#4})$);
\coordinate (WheelRL) at ($ (#1, #2) + ({-sin(#3)*#4}, {cos(#3)*#4})$);
\coordinate (WheelRR) at ($ (#1, #2) + ({-sin(#3)*-#4}, {cos(#3)*-#4})$);

\def\WheelWidth{0.06}
\def\WheelHeight{0.125}

\DrawWheel{(WheelFR)}{#3-20}{\WheelWidth}{\WheelHeight}
\DrawWheel{(WheelFL)}{#3-20}{\WheelWidth}{\WheelHeight}
\DrawWheel{(WheelRL)}{#3}{\WheelWidth}{\WheelHeight}
\DrawWheel{(WheelRR)}{#3}{\WheelWidth}{\WheelHeight}


}

==> figures/tikz/draw_wheel.tex <==
% This file defines the draw wheel command

\newcommand{\DrawWheel}[4]{
% #1 Wheel center coordinate
% #2 Wheel center y
% #3 Wheel theta
% #4 Wheel half width
% #5 Wheel half length

\coordinate (CornerFR) at ($ #1 + ({cos(#2)*#4-sin(#2)*-#3}, {sin(#2)*#4+cos(#2)*-#3})$);
\coordinate (CornerFL) at ($ #1 + ({cos(#2)*#4-sin(#2)*#3}, {sin(#2)*#4+cos(#2)*#3})$);
\coordinate (CornerRL) at ($ #1 + ({cos(#2)*-#4-sin(#2)*#3}, {sin(#2)*-#4+cos(#2)*#3})$);
\coordinate (CornerRR) at ($ #1 + ({cos(#2)*-#4-sin(#2)*-#3}, {sin(#2)*-#4+cos(#2)*-#3})$);

\draw[fill=black,very thick] (CornerFL) -- (CornerFR) -- (CornerRR) -- (CornerRL) -- cycle;

}
